Computational model of sphingolipids metabolism: a case study of Alzheimer's disease

Background: Sphingolipids - as suggested by the prefix in their name - are mysterious molecules, which play surprisingly various roles in opposable cellular processes, like autophagy, apoptosis, proliferation and differentiation. Recently they have been also recognized as important messengers in cellular signalling pathways. More importantly, sphingolipid metabolism disorders were observed in various pathological conditions such as cancer and neurodegeneration. Results: Existing formal models of sphingolipids metabolism concentrates mostly on de novo ceramide synthesis or restrict their focus to biochemical transformations of a particular subspecies. We propose first comprehensive computational model of sphingolipid metabolism in human tissue. In contrast to previous approaches we explicitly model compartmentalization what allows emphasizing the differences among individual organelles. Conclusions: Presented here model was validated by means of recently proposed model analysis technics allowing for detection of most sensitive and experimentally non-identifiable parameters and determination of main sources of model variance. Moreover, we demonstrate the utility of the model for the study of molecular processes underlying Alzheimer's disease.

==> glossary.tex <==
\RequirePackage[toc,style=longheader,nonumberlist]{glossaries}
%====GLOSSARIES DEFS============================================================
% glossaries definitions and associated auxilary commands
\makeglossaries
% TODO ungroup by letter if possible
%====header=============================
\renewcommand{\glossaryname}{Abbreviations}
\renewcommand{\entryname}{Abbreviation}
\renewcommand{\descriptionname}{Meaning}
% \renewcommand{\pagelistname}{Page}
\renewcommand{\glossaryheader}{
\bfseries\entryname & \bfseries\descriptionname \\%& \bfseries\pagelistname\\
& \\%& \\
\endhead}
%====width=============================
\setlength{\glsdescwidth}{0.6\textwidth}
\renewcommand*{\glsgroupskip}{}
%\setlength{\glspagelistwidth}{0.1\textwidth}
%====entries display====================
%\defglsdisplay{#1#4}
%\defglsdisplayfirst{\dfntxt{#2}} %(#1#4)}
%====entries============================
%====ABBREVIATIONS==============================================================
%\newglossaryentry{abbr:}{name={},
%description={}}
%beta -amyloid
\newglossaryentry{abbr:ACDase}{name={ACDase},description={Acidic Ceramidase}}
\newglossaryentry{abbr:AD}{name={AD},description={Alzheimer's Disease}}
\newglossaryentry{abbr:AlkCDase}{name={AlkCDase},description={Alkaline Ceramidase}}
\newglossaryentry{abbr:AlkCDase2}{name={AlkCDase2},description={Alkaline Ceramidase 2}}
\newglossaryentry{abbr:AlkCDase3}{name={AlkCDase3},description={Alkaline Ceramidase 3}}
\newglossaryentry{abbr:aSMase}{name={aSMase},description={Acid Sphingomyelinase}}
\newglossaryentry{abbr:Beta-GC}{name={Beta-GC},description={Glucosylceramidase }}
\newglossaryentry{abbr:BST}{name={BST},description={Biochemical Systems Theory}}
\newglossaryentry{abbr:C}{name={C},description={Cytoplasm}}
\newglossaryentry{abbr:CDase}{name={CDase},description={Ceramidase}}
\newglossaryentry{abbr:C1P}{name={C1P},description={Ceramide-1-Phosphate}}
\newglossaryentry{abbr:CER}{name={CER},description={Ceramide}}
\newglossaryentry{abbr:CERK}{name={CERK},description={Ceramide Kinase }}
\newglossaryentry{abbr:CerS}{name={CerS},description={Ceramide Synthase}}
\newglossaryentry{abbr:CERT}{name={CERT},description={Ceramide Transfer Protein }}
\newglossaryentry{abbr:CPTP}{name={CPTP},description={Ceramide-1-Phosphate Transfer Protein}}
\newglossaryentry{abbr:ER}{name={ER},description={Endoplasmatic Reticulum}}
\newglossaryentry{abbr:FAPP2}{name={FAPP2},description={Four-Phosphate Adaptor Protein 2 }}
\newglossaryentry{abbr:GA}{name={GA},description={Golgi Apparatus}}
\newglossaryentry{abbr:GACL}{name={GACL},description={Golgi Apparatus Cytoplasmic Leaflet}}
\newglossaryentry{abbr:GCS}{name={GCS},description={Ceramide glucosyltransferase }}
\newglossaryentry{abbr:GluCER}{name={GluCER},description={Glucosylceramide}}
\newglossaryentry{abbr:GSL}{name={GSL},description={Glycosphingolipid}}
\newglossaryentry{abbr:IM}{name={IM},description={Inner Membrane}}
\newglossaryentry{abbr:LacCerS}{name={LacCerS},description={Glucosylceramide beta-1,4-galactosyltransferase }}
\newglossaryentry{abbr:L}{name={L},description={Lysosome}}
\newglossaryentry{abbr:LTP}{name={LTP},description={Lipid-Transfer Proteins}}
\newglossaryentry{abbr:M}{name={M},description={Mmitocho}}
\newglossaryentry{abbr:MAL}{name={MAL},description={Mass Action Law kinetics}}
\newglossaryentry{abbr:MM}{name={MM},description={Michealis-Menten kinetics}}
\newglossaryentry{abbr:nSMase}{name={nSMase},description={Neutral Sphingomyelinase }}
\newglossaryentry{abbr:nSMase2}{name={nSMase2},description={Neutral Sphingomyelinase 2 }}
\newglossaryentry{abbr:NCDase}{name={NCDase},description={Neutral Ceramidase }}
\newglossaryentry{abbr:N}{name={N},description={Nucleus}}
\newglossaryentry{abbr:ODEs}{name={ODEs},description={Ordinary Differential Equations}}
\newglossaryentry{abbr:OM}{name={OM},description={Outer Membrane}}
\newglossaryentry{abbr:PAP2a}{name={PAP2a},description={Phosphatidic acid phosphatase type 2a }}
\newglossaryentry{abbr:PAP2b}{name={PAP2b},description={Phosphatidic acid phosphatase type 2b}}
\newglossaryentry{abbr:PAP2c}{name={PAP2c},description={Phosphatidic acid phosphatase type 2c}}
\newglossaryentry{abbr:S1P}{name={S1P},description={Sphingosine-1-Phosphate}}
\newglossaryentry{abbr:SDE}{name={SDE},description={Stochastic Differential Equations}}
\newglossaryentry{abbr:SK}{name={SK},description={Sphingosine Kinase}}
\newglossaryentry{abbr:SK1}{name={SK1},description={Sphingosine Kinase 1}}
\newglossaryentry{abbr:SK2}{name={SK2},description={Sphingosine Kinase 2}}
\newglossaryentry{abbr:SL}{name={SL},description={Sphingolipids}}
\newglossaryentry{abbr:SM}{name={SM},description={Sphingomyelin}}
\newglossaryentry{abbr:SMase}{name={SMase},description={Sphingomyelinase}}
\newglossaryentry{abbr:SMS}{name={SMS},description={Sphingomyelin Synthase}}
\newglossaryentry{abbr:SMS1}{name={SMS1},description={Sphingomyelin Synthase1}}
\newglossaryentry{abbr:SPH}{name={SPH},description={Sphingosine}}
\newglossaryentry{abbr:SPL1}{name={SPL1},description={Sphingosine 1-Phosphate Lyase 1}}
\newglossaryentry{abbr:SPP1}{name={SPP1},description={Sphingosine-1-Phosphate Phosphatase 1 }}
\newglossaryentry{abbr:SPP2}{name={SPP2},description={Sphingosine-1-Phosphate Phosphatase 2}}
\newglossaryentry{abbr:SPT}{name={SPT},description={Serine Palmitoyltransferase}}
%====COMMANDS===================================================================
% auxilary commands using glossaries entries
%====glossary interpretation cmds=======
\newcommand{\abbr}[1]{\gls{abbr:#1}}
\newcommand{\abbrdesc}[1]{\glsentrydesc{abbr:#1}}
\newcommand{\abbrdfn}[1]{\emph{\abbrdesc{#1}}}

